The braid group of a necklace

We show several geometric and algebraic aspects of a necklace: a link composed with a core circle and a series of circles linked to this core. We first prove that the fundamental group of the configuration space of necklaces (that we will call braid group of a necklace) is isomorphic to the braid group over an annulus quotiented by the square of the center. We then define braid groups of necklaces and affine braid groups of type A in terms of automorphisms of free groups and characterize these automorphisms among all automorphisms of free groups. In the case of affine braid groups of type A such representation is faithful.

==> pic-circles-08a.tex <==
\begin{tikzpicture}[scale=0.6]

\draw[ultra thick] (0,0) ..controls(1.5,2).. (0,4);
\draw[ultra thick] (1.5,0) ..controls(0,2).. (1.5,4);

\fill(0.75,1.05) circle(4pt);
\fill(0.75,2.95) circle(4pt);

\begin{scope}[xshift=4cm]
  \draw[ultra thick] (0,0) -- (0,4);
  \draw[ultra thick] (1.5,0) -- (1.5,4);
\end{scope}

\draw[<->,>=latex,ultra thick,blue] (1.5,2)--(3.5,2);

\end{tikzpicture}
